SMS-WSJ: Database, performance measures, and baseline recipe for multi-channel source separation and recognition

We present a multi-channel database of overlapping speech for training, evaluation, and detailed analysis of source separation and extraction algorithms: SMS-WSJ -- Spatialized Multi-Speaker Wall Street Journal. It consists of artificially mixed speech taken from the WSJ database, but unlike earlier databases we consider all WSJ0+1 utterances and take care of strictly separating the speaker sets present in the training, validation and test sets. When spatializing the data we ensure a high degree of randomness w.r.t. room size, array center and rotation, as well as speaker position. Furthermore, this paper offers a critical assessment of recently proposed measures of source separation performance. Alongside the code to generate the database we provide a source separation baseline and a Kaldi recipe with competitive word error rates to provide common ground for evaluation.

==> asr_table.tex <==
$s$       &   5.59 &   6.40 &   5.87 &  6.92 \\
&$x^{(\mathrm{early})}_0$   &  12.75 &   5.96 &   7.07 &  7.52 \\
&$x^{(\mathrm{early})}_1$   &  13.75 &   6.19 &   6.61 &  7.50 \\
&$x_0$     &  42.22 &  19.53 &   7.60 &  9.55 \\
&$x_1$     &  42.22 &  19.51 &   7.43 &  9.35 \\
&$x_0+n_0$ &  47.51 &  24.38 &  11.80 &  8.93 \\
&$x_1+n_1$ &  47.91 &  23.93 &  12.20 &  8.69 \\
